STEERING: Stein Information Directed Exploration for Model-Based Reinforcement Learning

Directed Exploration is a crucial challenge in reinforcement learning (RL), especially when rewards are sparse. Information-directed sampling (IDS), which optimizes the information ratio, seeks to do so by augmenting regret with information gain. However, estimating information gain is computationally intractable or relies on restrictive assumptions which prohibit its use in many practical instances. In this work, we posit an alternative exploration incentive in terms of the integral probability metric (IPM) between a current estimate of the transition model and the unknown optimal, which under suitable conditions, can be computed in closed form with the kernelized Stein discrepancy (KSD). Based on KSD, we develop a novel algorithm \algo: \textbf{STE}in information dir\textbf{E}cted exploration for model-based \textbf{R}einforcement Learn\textbf{ING}. To enable its derivation, we develop fundamentally new variants of KSD for discrete conditional distributions. {We further establish that {\algo} archives sublinear Bayesian regret, improving upon prior learning rates of information-augmented MBRL.} Experimentally, we show that the proposed algorithm is computationally affordable and outperforms several prior approaches.

==> s1_intro.tex <==
 \section{Introduction} 

 We will start with hitting the exploration problem in reinforcement leraning 

 PSRL has imersed as one of the most succeful algorithm in reinforcement learning, then drawbacks of PSRL, which has been pointed by existing works,
 


 Then Botao's IDS, and then drawbacks of IDS,

 There are other methods, we can do reward shaping, and ther is no theory, 

 In this work, we take a different IPM based approach, which has the capabilituy to enable sampling distance to optimal, but there are challenges associated with this approach, which we addressed int hsi work. 

 And then contributions, 

 Related works, separate...

 PSRL based methods

 IDS based methods

 Stein Discrepency

 % Question: Can we develop a computationally tractable posterior sampling-based RL algorithm which exhibits efficient directed exploration? 
  
        Reinforcement learning (RL) has shown great success in solving sequential decision-making problems under uncertainty [\blue{CITE}]. The objective of an RL agent is to maximize the long-term total reward over time. However, in most of the practical scenarios \citep{mnih_atari}, the true dynamics and reward structure of the environment are unknown to agents, which requires an agent to learn about the environment to eventually make good decisions. This leads to the exploration-exploitation dilemma \citep{sutton1998reinforcement} - where an agent needs to trade-off exploring to reduce uncertainty about the environment by exploiting the current best estimate of cumulative returns. {The focus of this work is to develop computationally tractable exploration incentives for model-based RL (MBRL) that alleviate the limitations of prior approaches.}
        
        Most RL algorithms fall into two categories: \emph{model-free} \citep{schulman2017proximal, mnih_qlearn, haarnoja2018soft,lillicrap_ddpg} and \emph{model-based} \citep{pmlr-v139-fan21b, deisenroth2011pilco, chua2018deep, janner2019trust}. In model-free approaches, the agent learns direct policy mapping from states to action with approximate dynamic programming methods. In contrast, in model-based approaches, an agent learns the approximate model of the environment itself and trains a policy under the learned dynamics. Recently, probabilistic model-based RL algorithms have shown superior performance in practice relative to their model-free counterparts, despite the strong conceptual guarantees for model-free approaches \citep{janner2019trust}. 
        
        To understand why this may be so, it's important to assess the convergence criteria of RL methods: Probably approximate correct (PAC) bounds \citep{Valiant}, Frequentist regret \citep{jin2018q, jin2020provably}, Bayesian regret \citep{osband2013}, Mistake (MB) Bound \citep{Littlestone}, KWIK (Knows What It Knows) \citep{Lihong} $\&$ convergence in various distributional metrics \citep{amortila2020distributional, borkar2002risk, Chakraborty_ksrl, chowdhury2019online} all exist. A crucial challenge lies in deciding the optimal selection criteria to evaluate the algorithm's computational and statistical efficiency. Rather than comment on the specific merit of a particular convergence criterion as a motivation for our restriction of focus to Bayesian regret, we note a few of its salient attributes: it imposes minimal requirements on access to a generative model underlying state transitions  \citep{osband17a, osband2013, osband2014model}, and respects the inherent uncertainty associated with the optimal policy, rather than supposing that it can be effectively captured by confidence sets based on a few moment-based estimates of the transition dynamics, which can lead to undesirable behavior in the presence of sparse rewards \citep{jin2020provably, yang2020reinforcement, zanette2020frequentist}.
        
         To encapsulate the inherent uncertainty present in the optimal policy, one may augment notions of regret to quantify distance to the optimal occupancy measure or other information-theoretic quantities \citep{russo2018learning,hao2022regret}. That this is advantageous may be seen by honing in on the sparse reward setting: consider the traditional definition of regret $\mathbb{E}[V^{*}(s) - V^{k}(s)]$ for any $k^{th}$ episode in an environment with near-zero rewards. Suppose one policy incorporates exploration based on a distributional estimate of the environment, whereas the other only consider moments of the distribution of returns, such as UCB \citep{lai1985asymptotically}. In this case, the traditional notion of regret may not encourage exploration in a way that yields increased state-space coverage, as the value distribution for this case would be near-null. This issue is well-documented in the bandit setting  \citep{thompson_tutorial}. Hence, there is an intrinsic motivation to consider augmentations of regret that are well-calibrated to the inherent uncertainty of the optimal policy. Motivated by \citep{russo2018learning,hao2022regret}, we consider convergence criteria from information theory and Bayesian inference to define an appropriate notion of regret.
        	
	  \begin{table}[t]
		  \centering
		  \resizebox{0.48\textwidth}{!}{\begin{tabular}{|c|c|c|c|c|}
				  \hline
				  \hline
				  \textbf{Refs} & \textbf{IR} & \textbf{IR Type} & \textbf{Bayes Regret}  & \textbf{Priori free/Implementable}\\ \hline
				  PSRL \citep{osband2013}        &    $\times$        &    \textemdash         &  $\tilde{ \mathcal{O}}( \sqrt{H^3S^2AK})$     & Yes/Yes \\ 
				  \hline[1-2]
				  PSRL2 \citep{osband17a}          &    $\times$       &  \textemdash      & $\tilde{\mathcal{O}}( \sqrt{H^3SAK})$           & Yes/Yes \\ \hline
				  TSDE \citep{ouyang2017control}     &    $\times$       &        \textemdash      & $\tilde{\mathcal{O}}( \sqrt{H^3S^2AK})$ & Yes/Yes   \\ \hline
				%  General PSRL \citep{agrawal2017optimistic}        &    $\times$      &          \textemdash      &  $\tilde{\mathcal{O}}(DS \sqrt{AT})$    \\ \hline
				  IDS-RL1* \citep{https://doi.org/10.48550/arxiv.1911.09724}      &    \checkmark            &         {Mutual Inf.}        & $\tilde{ \mathcal{O}}(\sqrt{H^3 SAK})$ & No/Yes        \\ \hline
				  IDS-RL2 \citep{hao2022regret}      &    \checkmark           &         {Mutual Inf.}     & $\tilde{ \mathcal{O}}(\sqrt{H^4 S^3 A^2 K})$  & Yes/No  \\ \hline
      \rowcolor{LightCyan}
				  {\algo} (\textbf{This work})          &    \checkmark     &      {Stein Dist.}             &   $\tilde{ \mathcal{O}}(\sqrt{H^4 S^2A K})$ & Yes/Yes \\ \hline
                  {{Minmax Lower Bound}}          &    -     &      \textemdash       &   $\tilde{ \mathcal{O}}(\sqrt{H^3 SA K})$ & NA\\ \hline
				  \end{tabular}}
		  % 
		  \caption{IR denotes Information Regularization. This table compares the Bayes regret (cf. \eqref{bayesian_Regret}) achieved and whether or not it considers the Information directed efficient exploration. Our {\algo} algorithm is able to achieve improved Bayes regret with Stein-Information directed sampling {(*denotes that the result only hold for specific Dirichlet prior with distribution-specific assumptions).} }\label{table_intro}% 
		  \end{table}
		  
        To understand the exact manner in which these modifications are incorporated into model-based RL (MBRL), we contrast them with the model-free setting. In such settings, incorporating exploration bonuses is well-established \citep{jin2020provably,eysenbach_entropy,liu_entropy,zafarali_entropy}, either in the form of augmenting the reward, the value function \citep{jin2018q,osband2019deep}, or the policy gradient \citep{gelfand1991recursive,raginsky2017non}. However, such methods sample uniformly with respect to a value or policy rather than in pursuit of reducing the estimation error to the optimal transition dynamics, which can yield spurious behavior \citep{weerakoon_sparse, shyam_sparse}. By contrast, information-theoretic regularisation in model-based RL is an active area of research. Empirical advancements based on intrinsic curiosity \citep{burda_curiosity,pathak_curiosity}, i.e., modifying the sampling probabilities driven by uncertainty estimates in the transition dynamics or forward model prediction error, can improve performance in practice but lack conceptual guarantees. 
        
        To substantiate these approaches conceptually, the resultant algorithms have recently been rewritten in a way that their performance can be quantified by information-theoretic or Bayesian regret \citep{lu_info, vanroy_bit}, under a specific choice of Dirichlet priors for the transition model, inspired by earlier work on bandits \citep{russo_info}. Extensions that alleviate any requirements on the prior for MBRL also exist based upon the development of a surrogate environment estimation procedure via rate-distortion theory   \citep{hao2022regret}. Unfortunately, the resultant algorithm requires estimating the KL divergence with respect to the true transition distribution, which in general, cannot be evaluated. This issue can be partially addressed by instead optimizing the evidence lower-bound (ELBO) \citep{achiam_lb}, but exhibits exponential dependence on the mutual information with respect to the optimal occupancy measure \citep{ozair_wasserstein}. Related approaches replace mutual information by Bregman divergence; however, this necessitates inverting a Fisher information matrix per step which can be computationally costly \citep{Lattimore_minmax, Zimmert_info}.
        Hence, previous efforts to incorporate information-theoretic bonuses in MBRL either impose restrictive assumptions on the prior or yield computationally heavy objectives whose algorithmic solutions exhibit scalability problems. This motivates us to pose the following question:
        
        \emph{Can we develop a computationally tractable posterior sampling-based RL algorithm that exhibits efficient directed exploration? }

            %    \emph{Is it possible to achieve sublinear Bayesian regret for IDS with computationally tractable updates without restrictions on the prior or sampling oracle?}

        We provide an affirmative answer to this question by introducing the distributional distance between the estimated and true transition dynamics with Integral probability metrics (IPM) \citep{sriperumbudur2012empirical} to characterise a notion of information-gain.  We introduced a distributional regret to tackle the above challenges. Specifically, assuming the transition distribution to lie in the Stein class, we employ Stein's identity \citep{efron1973stein,james1992estimation} to quantify the distribution divergence between the true (unknown) and estimated transitions in closed-form using Kernelized Stein discrepancy (KSD) \citep{gorham2015measuring, liu2016kernelized, hawkins2022online}, which alleviates a major drawback of prior-approaches of requiring access to the true transition. Thereby we introduce the Stein-information ratio, which may be seen as a modification of the information ratio in \citep{russo2018learning,vanroy_bit}, and incentivizes exploration in a directed manner. Doing so permits us to derive the best-known prior-free Bayesian regret bounds. A key point of departure in our analysis is that we replace the distributional distance between the current transition estimate and the optimal by the score function of the target, which can be estimated in practice via KSD. This step alleviates the costly sample complexity required to estimate mutual information which appears in alternate methodologies. Towards this end, we also develop the first KSD for conditional discrete distributions and employ it in tabular RL settings. The end result improves the best-known regret bounds from $\mathcal{\tilde{O}}(H^2SA \sqrt{SK}) \rightarrow \mathcal{\tilde{O}}(H^2 \sqrt{SAK})$. Our main contributions, then, are as follows
        \begin{list}{$\rhd$}{\topsep=0.ex \leftmargin=0.2in \rightmargin=0.in \itemsep =0.0in}
             \item we formalize the setting of model-based episodic RL with Bayesian regret incorporating a notion of distance to the ground-truth MDP with KSD;
             %
            \item we introduce Discrete Conditional KSD in tabular RL for the first time, and use it to analyze distributional distance, which relaxes the requirement of accessing the true transition dynamics for evaluating an exploration incentive. Through this definition, introduce a specific exploration-incentivized modification of posterior sampling which we call Stein Information Directed Sampling (SIDS) (Algorithm \ref{alg:MPC-PSRL}) ;
            %
            \item we establish prior-free Bayesian regret bounds for SIDS that are sublinear both in the number of episodes experienced and the dimension of the state-action space with distributional divergences thereby improving the best known prior-free Bayesian regret in \citep{hao2022regret}
            \item we develop a key novel connection between the information-directed sampling and sparse reward RL and experimentally demonstrate that SIDS achieves superior performance in terms of cumulative regret over prior approaches.
\end{list}

